Parameter estimation on gravitational waves from neutron-star binaries with spinning components

Inspiraling binary neutron stars are expected to be one of the most significant sources of gravitational-wave signals for the new generation of advanced ground-based detectors. We investigate how well we could hope to measure properties of these binaries using the Advanced LIGO detectors, which began operation in September 2015. We study an astrophysically motivated population of sources (binary components with masses $1.2~\mathrm{M}_\odot$--$1.6~\mathrm{M}_\odot$ and spins of less than $0.05$) using the full LIGO analysis pipeline. While this simulated population covers the observed range of potential binary neutron-star sources, we do not exclude the possibility of sources with parameters outside these ranges; given the existing uncertainty in distributions of mass and spin, it is critical that analyses account for the full range of possible mass and spin configurations. We find that conservative prior assumptions on neutron-star mass and spin lead to average fractional uncertainties in component masses of $\sim 16\%$, with little constraint on spins (the median $90\%$ upper limit on the spin of the more massive component is $\sim 0.7$). Stronger prior constraints on neutron-star spins can further constrain mass estimates, but only marginally. However, we find that the sky position and luminosity distance for these sources are not influenced by the inclusion of spin; therefore, if LIGO detects a low-spin population of BNS sources, less computationally expensive results calculated neglecting spin will be sufficient for guiding electromagnetic follow-up.

==> header.tex <==
\usepackage{natbib}
\bibliographystyle{plainnat}

==> posttitle.tex <==
\author{Ben Farr}
\affil{Enrico Fermi Institute, University of Chicago, Chicago, IL 60637, USA}
\email{farr@uchicago.edu}
 
\author{Christopher P. L. Berry and Will M. Farr and
        Carl-Johan Haster and Hannah Middleton}
\affil{School of Physics \& Astronomy, University of Birmingham, Birmingham, B15 2TT, UK}
 
\author{Kipp Cannon}
\affil{Canadian Institute for Theoretical Astrophysics, 60 St. George Street, University of Toronto, Toronto, Ontario, M5S 3H8, Canada}

\author{Philip B. Graff\altaffilmark{1}}
\affil{Department of Physics, University of Maryland--College Park, College Park, MD 20742, USA}
\altaffiltext{1}{Gravitational Astrophysics Lab, NASA Goddard Space Flight Center, Greenbelt, MD 20771, USA}
 
\author{Chad Hanna}
\affil{The Pennsylvania State University, University Park, PA 16802, USA}
 
\author{Ilya Mandel}
\affil{School of Physics \& Astronomy, University of Birmingham, Birmingham, B15 2TT, UK}
 
\author{Chris Pankow}
\affil{Leonard E. Parker Center for Gravitation, Cosmology, and Astrophysics, University of Wisconsin--Milwaukee, Milwaukee, WI 53201, USA}
 
\author{Larry R. Price}
\affil{LIGO Laboratory, California Institute of Technology, Pasadena, CA 91125, USA}

 \author{Trevor Sidery}
\affil{School of Physics \& Astronomy, University of Birmingham, Birmingham, B15 2TT, UK}
 
\author{Leo P. Singer}
\affil{Astrophysics Science Division, NASA Goddard Space Flight Center, Code 661, Greenbelt, MD 20771, USA}
 
\author{Alex L. Urban}
\affil{Leonard E. Parker Center for Gravitation, Cosmology, and Astrophysics, University of Wisconsin--Milwaukee, Milwaukee, WI 53201, USA}
 
\author{Alberto Vecchio and John Veitch}
\affil{School of Physics \& Astronomy, University of Birmingham, Birmingham, B15 2TT, UK}
 
\author{Salvatore Vitale}
\affil{Massachusetts Institute of Technology, 185 Albany St, Cambridge, MA 02139, USA}

